CUNI systems for WMT21: Multilingual Low-Resource Translation for Indo-European Languages Shared Task

This paper describes Charles University submission for Multilingual Low-Resource Translation for Indo-European Languages shared task at WMT21. We competed in translation from Catalan into Romanian, Italian and Occitan. Our systems are based on shared multilingual model. We show that using joint model for multiple similar language pairs improves upon translation quality in each pair. We also demonstrate that chararacter-level bilingual models are competitive for very similar language pairs (Catalan-Occitan) but less so for more distant pairs. We also describe our experiments with multi-task learning, where aside from a textual translation, the models are also trained to perform grapheme-to-phoneme conversion.

==> Makefile <==
SHELL=bash
MAINFILE=emnlp2021
all: $(MAINFILE).pdf $(MAINFILE)-sources.zip

$(MAINFILE)-sources.zip: $(MAINFILE).pdf $(MAINFILE).bbl
	zip -r $(MAINFILE)-sources.zip * -x .git/* .git/**\* *.pdf *.txt *.log *.aux *.blg *.out

$(MAINFILE).pdf:
	pdflatex $(MAINFILE).tex

$(MAINFILE).aux: $(MAINFILE).pdf

$(MAINFILE).bbl: $(MAINFILE).aux
	bibtex $(MAINFILE).aux
	pdflatex $(MAINFILE).tex
	pdflatex $(MAINFILE).tex

clean:
	rm -f *.{log,aux,blg,out,tmp}

clean_all:
	rm -f *.{log,aux,blg,out,tmp,bbl,zip}

